Development and characterization of a dispersion-encoded method for low-coherence interferometry

This work discusses an extension to conventional low-coherence interferometry by the introduction of dispersion-encoding. The extension facilitates the measurement of surface height profiles with sub-nm resolution. The selection of a dispersive element for encoding allows for tuning of the axial measurement range and resolution of the setup. The approach is theoretically designed and implemented for applications such as surface profilometry, the characterization of polymeric cross-linking and as a tool for the determination of layer thicknesses in thin-film processing. During the characterization of the implemented setup, it was shown that an axial measurement range of 79.91 $\mu m$ with a resolution of 0.1 nm was achievable in the evaluation of surface profiles. Simultaneously, profiles of up to 1.5 mm length could be obtained without the need for mechanical scanning. This marked a significant improvement in relation to state-of-the-art technologies in terms of dynamic range. It was also shown that axial and lateral measurement range can be decoupled partially. Additionally, functional parameters such as surface roughness were characterized with the same tool. The characterization of the degree of polymeric cross-linking was performed as a function of the refractive index. Here, the refractive index could be acquired in a spatially-resolved manner with an index resolution of down to $3.36 \pm 10^{-5}$. This was achieved by the development of a novel mathematical analysis approach. For the acquisition of layer thicknesses of thin-films, an advanced setup was developed which could be used to characterize the thickness thin-films and its (flexible) substrate simultaneously.

==> chapters/additional/selbstst_ndigkeitserkl_rung_ch_taudt_inline.tex <==

Hiermit versichere ich, dass ich die vorliegende Arbeit ohne unzulässige Hilfe Dritter und ohne Benutzung anderer als der angegebenen Hilfsmittel angefertigt habe; die aus fremden Quellen direkt oder indirekt übernommenen Gedanken sind als solche kenntlich gemacht. Bei der Auswahl und Auswertung des Materials sowie bei der Herstellung des Manuskripts habe ich Unterstützungsleistungen von folgenden Personen erhalten: \textit{Ich habe im Rahmen dieser Arbeit Publikationen mit Co-Autoren entsprechend der Publikationsliste erarbeitet. Mir wurden außerdem Proben zur Verfügung gestellt von Herrn M. Hapich (Fa. Ametek GmbH/Taylor Hobson; Rauheitsnormale), Herr Philipp Hanke (Fa. Layertec GmbH; Spiegelsubstrat mit Beschichtung) sowie durch Herrn Prof.\,Dr.\,rer.\,nat.\,Stefan Braun (Westsächsische Hochschule Zwickau; 3\,nm Höhenstufe auf Si). Daneben habe ich keine Unterstützungsleistungen erhalten.}\\
\\
Weitere Personen waren an der geistigen Herstellung der vorliegenden Arbeit nicht beteiligt. Insbesondere habe ich nicht die Hilfe eines kommerziellen Promotionsberaters in Anspruch genommen. Dritte haben von mir weder unmittelbar noch mittelbar geldwerte Leistungen für Arbeiten erhalten, die im Zusammenhang mit dem Inhalt der vorgelegten Dissertation stehen.\\
\\
Die Arbeit wurde bisher weder im Inland noch im Ausland in gleicher oder ähnlicher Form einer anderen Prüfungsbehörde vorgelegt und ist auch noch nicht veröffentlicht worden.\\
\\
Mir ist bekannt, dass die Nichteinhaltung dieser Erklärung zum nachträglichen Entzug des Doktortitels führen kann.\\
\\
Ich bestätige, dass ich die Promotionsordnung der Fakultät Elektrotechnik und Informationstechnik vom 08. August 1994 in der geänderten Fassung 12.05.2012 und die Änderungssatzung vom 18.06.2018 der Technischen Universität Dresden anerkenne.\\
\\
\\
\\
Zwickau, den 28.05.2020\\
\\
\\
\\
Christopher Taudt


